Statistical exponential families: A digest with flash cards

This document describes concisely the ubiquitous class of exponential family distributions met in statistics. The first part recalls definitions and summarizes main properties and duality with Bregman divergences (all proofs are skipped). The second part lists decompositions and related formula of common exponential family distributions. We recall the Fisher-Rao-Riemannian geometries and the dual affine connection information geometries of statistical manifolds. It is intended to maintain and update this document and catalog by adding new distribution items.

==> Dirichlet.tex <==
\section{Dirichlet distribution}

$B(\alpha)=\frac{\prod_{i=1}^k \Gamma(\alpha_i)}{\Gamma(\sum_{i=1}^k \alpha_i)}$

\begin{tabular}{|c|c|}
	\hline
	%
	PDF expression  & $f(x;\alpha_1, ..., \alpha_k) = \frac{1}{B(\alpha) \prod_{i=1}^k x_i^{\alpha_i-1}}$ with $\alpha_i>0$ and $\sum_{i=1}^k \alpha_i=1$\\
	%
	\hline
	\hline
	%
	% http://ilab.usc.edu/wiki/index.php/Dirichlet_Kullback-Leibler
	Kullback-Leibler divergence &
	$D_{\mathrm{KL}}(f_P\|f_Q) = \log\frac{B(\alpha_P)}{B(\alpha_Q)} +\sum_{i=1}^k (\alpha_{i,P}-\alpha_{i,Q})(\digamma(\alpha_i)-\digamma(\alpha)))$ \\
	%
	\hline
	%
	MLE &
	\\
	%
	\hline
	\hline
	%
	Source parameters  & $\mathbf{\Lambda} = $ \\
	%
	\hline
	%
	Natural parameters & $\mathbf{\Theta} = $ \\
	%
	\hline
	%
	Expectation parameters & $\mathbf{H} = $ \\
	%
	\hline
	\hline
	%
	$\mathbf{\Lambda} \rightarrow \mathbf{\Theta}$ &
	$\mathbf{\Theta} = $ \\
	%
	\hline
	%
	$\mathbf{\Theta} \rightarrow \mathbf{\Lambda}$ &
	$\mathbf{\Lambda} =  $  \\
	%
	\hline
	%
	$\mathbf{\Lambda} \rightarrow \mathbf{H}$ &
	$\mathbf{H} =  $ \\
	%
	\hline
	%
	$\mathbf{H} \rightarrow \mathbf{\Lambda}$ &
	$\mathbf{\Lambda} = $  \\
	%
	\hline
	%
	$\mathbf{\Theta} \rightarrow \mathbf{H}$ &
	$\mathbf{H} = $ \\
	%
	\hline
	%
	$\mathbf{H} \rightarrow \mathbf{\Theta}$ &
	$\mathbf{\Theta} = $  \\
	%
	\hline
	\hline
	%
	Log normalizer &
	$ F(\mathbf{\Theta}) = \sum_{i=1}^k \log\Gamma(\theta_i)  - \log\Gamma(\sum_{i=1}^k \theta_i) $  \\
	%
	\hline
	%
	Gradient log normalizer & $
	\nabla F(\mathbf{\Theta}) = $  \\
	%
	\hline
	%
	G &
	$G(\mathbf{H}) = $  \\
	%
	\hline
	%
	Gradient G &
	$\nabla G(\mathbf{H}) = $  \\
	%
	\hline
	\hline
	%
	Sufficient statistics & $ t(x) = (\log x_1, ..., \log x_k) $  \\
	%
	\hline
	%
	Carrier measure & $ k(x) =  \prod_{i=1}^k \frac{1}{x_i}$  \\
	%
	\hline
\end{tabular}

==> InverseGaussian.tex <==
\section{Inverse Gaussian distribution}

\begin{tabular}{|c|c|}
	\hline
	%
	PDF expression  & $f(x;) = $ \\
	%
	\hline
	\hline
	%
	Kullback-Leibler divergence &
	$D_{\mathrm{KL}}(f_P\|f_Q) = $ \\
	%
	\hline
	%
	MLE &
	\\
	%
	\hline
	\hline
	%
	Source parameters  & $\mathbf{\Lambda} = $ \\
	%
	\hline
	%
	Natural parameters & $\mathbf{\Theta} = $ \\
	%
	\hline
	%
	Expectation parameters & $\mathbf{H} = $ \\
	%
	\hline
	\hline
	%
	$\mathbf{\Lambda} \rightarrow \mathbf{\Theta}$ &
	$\mathbf{\Theta} = $ \\
	%
	\hline
	%
	$\mathbf{\Theta} \rightarrow \mathbf{\Lambda}$ &
	$\mathbf{\Lambda} =  $  \\
	%
	\hline
	%
	$\mathbf{\Lambda} \rightarrow \mathbf{H}$ &
	$\mathbf{H} =  $ \\
	%
	\hline
	%
	$\mathbf{H} \rightarrow \mathbf{\Lambda}$ &
	$\mathbf{\Lambda} = $  \\
	%
	\hline
	%
	$\mathbf{\Theta} \rightarrow \mathbf{H}$ &
	$\mathbf{H} = $ \\
	%
	\hline
	%
	$\mathbf{H} \rightarrow \mathbf{\Theta}$ &
	$\mathbf{\Theta} = $  \\
	%
	\hline
	\hline
	%
	Log normalizer &
	$ F(\mathbf{\Theta}) = -2\sqrt{\theta_1\theta_2}-\frac{1}{2}\log\theta_2 +\frac{1}{2}\log\pi $  \\
	%
	\hline
	%
	Gradient log normalizer & $
	\nabla F(\mathbf{\Theta}) = $  \\
	%
	\hline
	%
	G &
	$G(\mathbf{H}) = $  \\
	%
	\hline
	%
	Gradient G &
	$\nabla G(\mathbf{H}) = $  \\
	%
	\hline
	\hline
	%
	Sufficient statistics & $ t(x) = (-x,-\frac{1}{x})$  \\
	%
	\hline
	%
	Carrier measure & $ k(x) = x^{-\frac{3}{2}}$  \\
	%
	\hline
\end{tabular}

==> Lognormal.tex <==
\section{Lognormal distribution}

\begin{tabular}{|c|c|}
	\hline
	%
	PDF expression  & $f(x;) = $ \\
	%
	\hline
	\hline
	%
	Kullback-Leibler divergence &
	$D_{\mathrm{KL}}(f_P\|f_Q) = $ \\
	%
	\hline
	%
	MLE &  $\hat\mu=\frac{1}{n} \sum_{i=1}^n x_i$ $\hat\sigma=\sqrt{\frac{1}{n}\sum_{i=1}^n (\log x_i-\hat\mu)^2}$
	\\
	%
	\hline
	\hline
	%
	Source parameters  & $\mathbf{\Lambda} = $ \\
	%
	\hline
	%
	Natural parameters & $\mathbf{\Theta} = $ \\
	%
	\hline
	%
	Expectation parameters & $\mathbf{H} = $ \\
	%
	\hline
	\hline
	%
	$\mathbf{\Lambda} \rightarrow \mathbf{\Theta}$ &
	$\mathbf{\Theta} = $ \\
	%
	\hline
	%
	$\mathbf{\Theta} \rightarrow \mathbf{\Lambda}$ &
	$\mathbf{\Lambda} =  $  \\
	%
	\hline
	%
	$\mathbf{\Lambda} \rightarrow \mathbf{H}$ &
	$\mathbf{H} =  $ \\
	%
	\hline
	%
	$\mathbf{H} \rightarrow \mathbf{\Lambda}$ &
	$\mathbf{\Lambda} = $  \\
	%
	\hline
	%
	$\mathbf{\Theta} \rightarrow \mathbf{H}$ &
	$\mathbf{H} = $ \\
	%
	\hline
	%
	$\mathbf{H} \rightarrow \mathbf{\Theta}$ &
	$\mathbf{\Theta} = $  \\
	%
	\hline
	\hline
	%
	Log normalizer &
	$ F(\mathbf{\Theta}) = $  \\
	%
	\hline
	%
	Gradient log normalizer & $
	\nabla F(\mathbf{\Theta}) = $  \\
	%
	\hline
	%
	G &
	$G(\mathbf{H}) = $  \\
	%
	\hline
	%
	Gradient G &
	$\nabla G(\mathbf{H}) = $  \\
	%
	\hline
	\hline
	%
	Sufficient statistics & $ t(x) = $  \\
	%
	\hline
	%
	Carrier measure & $ k(x) = $  \\
	%
	\hline
\end{tabular}

==> Wishart.tex <==
\section{Wishart distribution}

$|x|$ denotes the determinant of matrix $x$.

\begin{tabular}{|c|c|}
	\hline
	%
	PDF expression  & $f(X;p,V) = \frac{|X|^{\frac{d-p-1}{2}}}{2^{\frac{dp}{2}}|V|^{\frac{d}{2}}\Gamma_p(\frac{d}{2})}\exp (-\frac{1}{2}\tr (V^{-1}X)) $ \\
	%
	\hline
	\hline
	%
	Kullback-Leibler divergence &
	$D_{\mathrm{KL}}(f_P\|f_Q) = $ \\
	%
	\hline
	%
	MLE &
	\\
	%
	\hline
	\hline
	%
	Source parameters  & $\mathbf{\Lambda} = $ \\
	%
	\hline
	%
	Natural parameters & $\mathbf{\Theta} = $ \\
	%
	\hline
	%
	Expectation parameters & $\mathbf{H} = $ \\
	%
	\hline
	\hline
	%
	$\mathbf{\Lambda} \rightarrow \mathbf{\Theta}$ &
	$\mathbf{\Theta} = $ \\
	%
	\hline
	%
	$\mathbf{\Theta} \rightarrow \mathbf{\Lambda}$ &
	$\mathbf{\Lambda} =  $  \\
	%
	\hline
	%
	$\mathbf{\Lambda} \rightarrow \mathbf{H}$ &
	$\mathbf{H} =  $ \\
	%
	\hline
	%
	$\mathbf{H} \rightarrow \mathbf{\Lambda}$ &
	$\mathbf{\Lambda} = $  \\
	%
	\hline
	%
	$\mathbf{\Theta} \rightarrow \mathbf{H}$ &
	$\mathbf{H} = $ \\
	%
	\hline
	%
	$\mathbf{H} \rightarrow \mathbf{\Theta}$ &
	$\mathbf{\Theta} = $  \\
	%
	\hline
	\hline
	%
	Log normalizer &
	$ F(\mathbf{\Theta}) = -\theta_1\log|\theta_2|+\theta_1 d\log 2$  \\
	%
	\hline
	%
	Gradient log normalizer & $
	\nabla F(\mathbf{\Theta}) = $  \\
	%
	\hline
	%
	G &
	$G(\mathbf{H}) = $  \\
	%
	\hline
	%
	Gradient G &
	$\nabla G(\mathbf{H}) = $  \\
	%
	\hline
	\hline
	%
	Sufficient statistics & $ t(x) = (\log |x|,-\frac{1}{2}x)$  \\
	%
	\hline
	%
	Carrier measure & $ k(x) = |x|^{-\frac{d+1}{2}} $  \\
	%
	\hline
\end{tabular}
